High [OIII]/[CII] surface brightness ratios trace early starburst galaxies

We study the impact of deviations from the Kennicutt-Schmidt relation (quantified by the `burstiness' parameter $\kappa_s$), gas metallicity ($Z$), and density ($n$) on the observed [OIII]88$\mu$m/[CII]158$\mu$m surface brightness ratios ($\Sigma_{[OIII]}/\Sigma_{[CII]}$) in nine galaxies at $z\approx6-9$. We first discuss possible biases in the measured $\Sigma_{[OIII]}/\Sigma_{[CII]}$ ratios by comparing the data with zoom-in cosmological simulations, and then use a Markov Chain Monte Carlo algorithm to derive the best fit values of ($\kappa_s, Z, n$). We find that (i) the strongest dependence of $\Sigma_{[OIII]}/\Sigma_{[CII]}$ is on $\kappa_s$; (ii) high ratios identify starburst galaxies with short gas depletion times ($t_{dep}=6-49\,\rm Myr$); (iii) a secondary dependence on density is found, with $\Sigma_{[OIII]}/\Sigma_{[CII]}$ anticorrelating with $n$ as a result of the lower [OIII] critical density, (iv) the ratio only weakly depends on $Z$. The nine galaxies are significantly enriched (Z=0.2-0.5 $Z_\odot$), and dense ($n=10^{1-3} {\rm cm}^{-3}$). This lends further support to the starburst scenario in which a rapid enrichment of the interstellar medium is expected.

==> pdflink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother


